A User-Centric, Privacy-Preserving, and Verifiable Ecosystem for Personal Data Management and Utilization

In the current paradigm of digital personalized services, the centralized management of personal data raises significant privacy concerns, security vulnerabilities, and diminished individual autonomy over sensitive information. Despite their efficiency, traditional centralized architectures frequently fail to satisfy rigorous privacy requirements and expose users to data breaches and unauthorized access risks. This pressing challenge calls for a fundamental paradigm shift in methodologies for collecting, storing, and utilizing personal data across diverse sectors, including education, healthcare, and finance. This paper introduces a novel decentralized, privacy-preserving architecture that handles heterogeneous personal information, ranging from educational credentials to health records and financial data. Unlike traditional models, our system grants users complete data ownership and control, allowing them to selectively share information without compromising privacy. The architecture's foundation comprises advanced privacy-enhancing technologies, including secure enclaves and federated learning, enabling secure computation, verification, and data sharing. The system supports diverse functionalities, including local computation, model training, and privacy-preserving data sharing, while ensuring data credibility and robust user privacy.

==> bibItems.tex <==
\bibitem{AWS-ECS}AWS, A. Amazon Elastic Container Service. , https://aws.amazon.com/ecs/
\bibitem{DIDs}DIDComm Decentralized Identifiers (DIDs). , https://www.w3.org/TR/did-core/
\bibitem{DIDComm}DIDComm DIDComm Messaging. , https://identity.foundation/didcomm-messaging/spec/v2.1/
\bibitem{alazab2024privacy}Alazab, M., Gadekallu, T., Pham, Q., Maddikunta, P., Bhattacharya, S., Piran, M. \& Hossain, M. Privacy and Security in Distributed Learning: A Review of Challenges, Solutions, and Open Research Issues. {\em IEEE Transactions On Industrial Informatics}. (2024), https://ieeexplore.ieee.org/document/10278413
\bibitem{ABAC}Amazon-AWS Attribute-Based Access Control (ABAC) for AWS. , https://aws.amazon.com/identity/attribute-based-access-control
\bibitem{AWSNitroEnclaves}Amazon.com AWS Nitro Enclaves: Create additional isolation to further protect highly sensitive data within EC2 instances. , https://aws.amazon.com/ec2/nitro/nitro-enclaves/
\bibitem{aslan2023}Aslan, Ö., Aktuğ, S., Ozkan-Okay, M., Yilmaz, A. \& Akin, E. A Comprehensive Review of Cyber Security Vulnerabilities, Threats, Attacks, and Solutions. {\em Electronics}. \textbf{12} (2023), https://www.mdpi.com/2079-9292/12/6/1333
\bibitem{whatIsNitro}AWS, A. What is AWS Nitro Enclaves?. , https://docs.aws.amazon.com/enclaves/latest/user/nitro-enclave.html
\bibitem{battiston2023}Battiston, I. \& Boncz, P. Improving Data Minimization through Decentralized Data Architectures. {\em ArXiv}. \textbf{2312.12923} (2023), https://arxiv.org/abs/2312.12923
\bibitem{ben2014succinct}Ben-Sasson, E., Chiesa, A., Tromer, E. \& Virza, M. Succinct non-interactive zero knowledge for a von Neumann architecture. {\em 23rd USENIX Security Symposium (USENIX Security 14)}. pp. 781-796 (2014)
\bibitem{bunz2018bulletproofs}B"unz, B., Bootle, J., Boneh, D., Poelstra, A., Wuille, P. \& Maxwell, G. Bulletproofs: Short proofs for confidential transactions and more. {\em 2018 IEEE Symposium On Security And Privacy (SP)}. pp. 315-334 (2018)
\bibitem{dataswift}Dataswift Dataswift - Personal Data Accounts. (Dataswift Ltd.,2023), https://dataswift.io/
\bibitem{digime}Digi.me digi.me - Your Data, Your Way. (digi.me Ltd.,2023), https://digi.me/
\bibitem{dwork2006differential}Dwork, C. Differential privacy. {\em International Colloquium On Automata, Languages, And Programming}. pp. 1-12 (2006)
\bibitem{databank}Fernández, M., Franch Tapia, A., Jaimunk, J., Martinez Chamorro, M. \& Thuraisingham, B. A Data Access Model for Privacy-Preserving Cloud-IoT Architectures. {\em Proceedings Of The 25th ACM Symposium On Access Control Models And Technologies}. pp. 191-202 (2020), https://doi.org/10.1145/3381991.3395610
\bibitem{groth2016size}Groth, J. On the size of pairing-based non-interactive arguments. {\em Annual International Conference On The Theory And Applications Of Cryptographic Techniques}. pp. 305-326 (2016)
\bibitem{latupeirissa2024}Latupeirissa, J., Dewi, N., Prayana, I., Srikandi, M., Ramadiansyah, S. \& Pramana, I. Transforming Public Service Delivery: A Comprehensive Review of Digitization Initiatives. {\em Sustainability}. \textbf{16}, 2818 (2024), https://www.mdpi.com/2071-1050/16/7/2818
\bibitem{meeco}Meeco Meeco: Enterprise Infrastructure for the Personal Data Economy. (https://www.meeco.me/), Accessed: 2024-12-03
\bibitem{mireshghallah2021privacy}Mireshghallah, F., Lundgren, M., Asghari, P., Ren, S., Kuzmanovic, A. \& Nilizadeh, S. Privacy-Preserving Machine Learning: Methods, Challenges, and Directions. {\em ArXiv Preprint ArXiv:2108.04417}. (2021)
\bibitem{databox}Mortier, R., Zhao, J., Crowcroft, J., Wang, L., Li, Q., Haddadi, H., Amar, Y., Crabtree, A., Colley, J., Lodge, T., Brown, T., McAuley, D. \& Greenhalgh, C. Personal Data Management with the Databox: What's Inside the Box?. {\em Proceedings Of The 2016 ACM Workshop On Cloud-Assisted Networking}. pp. 49-54 (2016), https://doi.org/10.1145/3010079.3010082
\bibitem{openpds}Openpds Openpds, Personal Data with Privacy. , https://openpds.media.mit.edu
\bibitem{personaldataio}PersonalData.IO Home - PersonalData.IO. (https://personaldata.io/en/home-en/), Accessed: 2024-12-03
\bibitem{ppds}Singh, B., Carminati, B. \& Ferrari, E. Privacy-Aware Personal Data Storage (P-PDS): Learning how to Protect User Privacy from External Applications. {\em IEEE Transactions On Dependable And Secure Computing}. \textbf{18}, 889-903 (2021)
\bibitem{Solid}Solid Solid: Your data, your choice.  (0), https://solidproject.org
\bibitem{wikipedia2021gdpr}Wikipedia contributors General Data Protection Regulation. (https://en.wikipedia.org/wiki/General_Data_Protection_Regulation,2021), Accessed: Mar 30, 2025
\bibitem{emre_codaspy}Yilmaz, E., T.Ji, Ayday, E. \& P.Li Genomic Data Sharing under Dependent Local Differential Privacy. {\em Proceedings Of ACM Conference On Data And Application Security And Privacy (CODASPY)}. (2022)


==> bibli.tex <==
\bibitem{10.1145/2810103.2813677}Fredrikson, M., Jha, S. \& Ristenpart, T. Model Inversion Attacks That Exploit Confidence Information and Basic Countermeasures. {\em Proceedings Of The 22nd ACM SIGSAC Conference On Computer And Communications Security}. pp. 1322-1333 (2015), https://doi.org/10.1145/2810103.2813677
\bibitem{linardatos}Linardatos, P., Papastefanopoulos, V. \& Kotsiantis, S. Explainable ai: A review of machine learning interpretability methods. {\em Entropy}. \textbf{23}, 18 (2020)
\bibitem{iris}Fisher, R. Iris. (UCI Machine Learning Repository,1988), DOI: https://doi.org/10.24432/C56C76
\bibitem{mushroom}Irvine, U. Mushroom. (UCI Machine Learning Repository,1987), DOI: https://doi.org/10.24432/C5959T
\bibitem{nursery}Rajkovic, V. Nursery. (UCI Machine Learning Repository,1997), DOI: https://doi.org/10.24432/C5P88W
\bibitem{adult}Becker, B. \& Kohavi, R. Adult. (UCI Machine Learning Repository,1996), DOI: https://doi.org/10.24432/C5XW20
\bibitem{breast}Mangasarian, O., Street, W. \& Wolberg, W. Breast Cancer Wisconsin (Diagnostic). (UCI Machine Learning Repository,1995), DOI: https://doi.org/10.24432/C5DW2B
\bibitem{german}Hofmann, H. Statlog (German Credit Data). (UCI Machine Learning Repository,1994), DOI: https://doi.org/10.24432/C5NC77
\bibitem{rigaki2020survey}Rigaki, M. \& Garcia, S. A survey of privacy attacks in machine learning. {\em ArXiv Preprint ArXiv:2007.07646}. (2020)
\bibitem{uci}Kelly, M., Longjohn, R. \& Nottingham, K. UCI Machine Learning Repository. (University of California, Irvine, School of Information,2023), https://archive.ics.uci.edu
\bibitem{bordes}Bordes, A., Ertekin, S., Weston, J. \& Bottou, L. Fast Kernel Classifiers with Online and Active Learning. {\em Journal Of Machine Learning Research}. \textbf{6}, 1579-1619 (2005), http://jmlr.org/papers/v6/bordes05a.html
\bibitem{beygelzimer}Beygelzimer, A., Hsu, D., Langford, J. \& Zhang, T. Agnostic active learning without constraints. {\em Advances In Neural Information Processing Systems}. \textbf{23} (2010)
\bibitem{selvaraju2017grad}Selvaraju, R., Cogswell, M., Das, A., Vedantam, R., Parikh, D. \& Batra, D. Grad-cam: Visual explanations from deep networks via gradient-based localization. {\em Proceedings Of The IEEE International Conference On Computer Vision}. pp. 618-626 (2017)
\bibitem{simonyan2013deep}Simonyan, K., Vedaldi, A. \& Zisserman, A. Deep inside convolutional networks: Visualising image classification models and saliency maps. {\em ArXiv Preprint ArXiv:1312.6034}. (2013)
\bibitem{zhou2016learning}Zhou, B., Khosla, A., Lapedriza, A., Oliva, A. \& Torralba, A. Learning deep features for discriminative localization. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 2921-2929 (2016)
\bibitem{cifar}Krizhevsky, A., Nair, V. \& Hinton, G. Cifar-10 (canadian institute for advanced research).  (2010), http://www.cs.toronto.edu/~kriz/cifar.html
\bibitem{lecun-mnisthandwrittendigit-2010}LeCun, Y. \& Cortes, C. MNIST handwritten digit database. (http://yann.lecun.com/exdb/mnist/,2010)
\bibitem{activethief}Pal, S., Gupta, Y., Shukla, A., Kanade, A., Shevade, S. \& Ganapathy, V. Activethief: Model extraction using active learning and unannotated public data. {\em Proceedings Of The AAAI Conference On Artificial Intelligence}. \textbf{34} pp. 865-872 (2020)
\bibitem{rudin2019stop}Rudin, C. Stop explaining black box machine learning models for high stakes decisions and use interpretable models instead. {\em Nature Machine Intelligence}. \textbf{1}, 206-215 (2019)
\bibitem{quinlan1986induction}Quinlan, J. Induction of decision trees. {\em Machine Learning}. \textbf{1}, 81-106 (1986)
\bibitem{delen2013measuring}Delen, D., Kuzey, C. \& Uyar, A. Measuring firm performance using financial ratios: A decision tree approach. {\em Expert Systems With Applications}. \textbf{40}, 3970-3983 (2013)
\bibitem{dovsilovic2018explainable}Došilović, F., Brčić, M. \& Hlupić, N. Explainable artificial intelligence: A survey. {\em 2018 41st International Convention On Information And Communication Technology, Electronics And Microelectronics (MIPRO)}. pp. 0210-0215 (2018)
\bibitem{holzinger2022explainable}Holzinger, A., Saranti, A., Molnar, C., Biecek, P. \& Samek, W. Explainable AI methods-a brief overview. {\em XxAI-Beyond Explainable AI: International Workshop, Held In Conjunction With ICML 2020, July 18, 2020, Vienna, Austria, Revised And Extended Papers}. pp. 13-38 (2022)
\bibitem{gepp2010business}Gepp, A., Kumar, K. \& Bhattacharya, S. Business failure prediction using decision trees. {\em Journal Of Forecasting}. \textbf{29}, 536-555 (2010)
\bibitem{1500165}Yao, Z., Liu, P., Lei, L. \& Yin, J. R-C4.5 decision tree model and its applications to health care dataset. {\em Proceedings Of ICSSSM '05. 2005 International Conference On Services Systems And Services Management, 2005.}. \textbf{2} pp. 1099-1103 Vol. 2 (2005)
\bibitem{yoo2012data}Yoo, I., Alafaireet, P., Marinov, M., Pena-Hernandez, K., Gopidi, R., Chang, J. \& Hua, L. Data mining in healthcare and biomedicine: a survey of the literature. {\em Journal Of Medical Systems}. \textbf{36} pp. 2431-2448 (2012)
\bibitem{chandra}Chandrasekaran, V., Chaudhuri, K., Giacomelli, I., Jha, S. \& Yan, S. Exploring Connections Between Active Learning and Model Extraction. {\em 29th USENIX Security Symposium (USENIX Security 20)}. pp. 1309-1326 (2020,8), https://www.usenix.org/conference/usenixsecurity20/presentation/chandrasekaran
\bibitem{NASSER20159192}Nasseri, A., Tucker, A. \& De Cesare, S. Quantifying StockTwits semantic terms’ trading behavior in financial markets: An effective application of decision tree algorithms. {\em Expert Systems With Applications}. \textbf{42}, 9192-9210 (2015), https://www.sciencedirect.com/science/article/pii/S0957417415005473
\bibitem{WU2006270}Wu, M., Lin, S. \& Lin, C. An effective application of decision tree to stock trading. {\em Expert Systems With Applications}. \textbf{31}, 270-274 (2006), https://www.sciencedirect.com/science/article/pii/S0957417405002137
\bibitem{1372413}Zekic-Susac, M., Sarlija, N. \& Bensic, M. Small business credit scoring: a comparison of logistic regression, neural network, and decision tree models. {\em 26th International Conference On Information Technology Interfaces, 2004.}. pp. 265-270 Vol.1 (2004)
\bibitem{10.1002/for.1153}Gepp, A., Kumar, K. \& Bhattacharya, S. Business failure prediction using decision trees. {\em Journal Of Forecasting}. \textbf{29}, 536-555 (2010), https://onlinelibrary.wiley.com/doi/abs/10.1002/for.1153
\bibitem{breiman1984classification}Breiman, L., Friedman, J., Stone, C. \& Olshen, R. Classification and Regression Trees. (Taylor & Francis,1984), https://books.google.com/books?id=JwQx-WOmSyQC
\bibitem{10.1145/3460120.3484575}Li, Z. \& Zhang, Y. Membership Leakage in Label-Only Exposures. {\em Proceedings Of The 2021 ACM SIGSAC Conference On Computer And Communications Security}. pp. 880-895 (2021), https://doi.org/10.1145/3460120.3484575
\bibitem{pmlr-v139-choquette-choo21a}Choquette-Choo, C., Tramer, F., Carlini, N. \& Papernot, N. Label-Only Membership Inference Attacks. {\em Proceedings Of The 38th International Conference On Machine Learning}. \textbf{139} pp. 1964-1974 (2021,7,18), https://proceedings.mlr.press/v139/choquette-choo21a.html
\bibitem{DBLP:journals/corr/abs-1912-00888}Lukas, N., Zhang, Y. \& Kerschbaum, F. Deep Neural Network Fingerprinting by Conferrable Adversarial Examples. {\em CoRR}. \textbf{abs/1912.00888} (2019), http://arxiv.org/abs/1912.00888
\bibitem{scikit-learn}Pedregosa, F., Varoquaux, G., Gramfort, A., Michel, V., Thirion, B., Grisel, O., Blondel, M., Prettenhofer, P., Weiss, R., Dubourg, V., Vanderplas, J., Passos, A., Cournapeau, D., Brucher, M., Perrot, M. \& Duchesnay, E. Scikit-learn: Machine Learning in Python. {\em Journal Of Machine Learning Research}. \textbf{12} pp. 2825-2830 (2011)
\bibitem{lime_github}Ribeiro, M. GitHub - marcotcr/lime: Lime: Explaining the predictions of any machine learning classifier.  (2016)
\bibitem{lowd}Lowd, D. \& Meek, C. Adversarial learning. {\em Proceedings Of The Eleventh ACM SIGKDD International Conference On Knowledge Discovery In Data Mining}. pp. 641-647 (2005)
\bibitem{azureExp}Azure, M. Model interpretability - Azure Machine Learning — learn.microsoft.com.  (2022), https://learn.microsoft.com/en-us/azure/machine-learning/how-to-machine-learning-interpretability?view=azureml-api-2
\bibitem{ibmExp}Cloud, I. Explaining transactions — ibm.com.  (2023), https://www.ibm.com/docs/en/cloud-paks/cp-data/3.5.0?topic=insights-explaining-transactions
\bibitem{owengame}Owen, G. Game theory. (Emerald Group Publishing,2013)
\bibitem{shapley}Shapley, L. Notes on the N-Person Game - I: Characteristic-Point Solutions of the Four-Person Game. (RAND Corporation,1951)
\bibitem{10.5555/3241094.3241142}Tramèr, F., Zhang, F., Juels, A., Reiter, M. \& Ristenpart, T. Stealing Machine Learning Models via Prediction APIs. {\em Proceedings Of The 25th USENIX Conference On Security Symposium}. pp. 601-618 (2016)
\bibitem{BARREDOARRIETA202082}Barredo Arrieta, A., Díaz-Rodríguez, N., Del Ser, J., Bennetot, A., Tabik, S., Barbado, A., Garcia, S., Gil-Lopez, S., Molina, D., Benjamins, R., Chatila, R. \& Herrera, F. Explainable Artificial Intelligence (XAI): Concepts, taxonomies, opportunities and challenges toward responsible AI. {\em Information Fusion}. \textbf{58} pp. 82-115 (2020), https://www.sciencedirect.com/science/article/pii/S1566253519308103
\bibitem{10.1145/2939672.2939778}Ribeiro, M., Singh, S. \& Guestrin, C. "Why Should I Trust You?": Explaining the Predictions of Any Classifier. {\em Proceedings Of The 22nd ACM SIGKDD International Conference On Knowledge Discovery And Data Mining}. pp. 1135-1144 (2016), https://doi.org/10.1145/2939672.2939778
\bibitem{ibm}Center, I. Explainable Artificial Intelligence (XAI). {\em IBM}. (2019), https://www.ibm.com/watson/explainable-ai
\bibitem{DBLP:journals/corr/abs-2009-01884}Aı̈vodji, U., Bolot, A. \& Gambs, S. Model extraction from counterfactual explanations. {\em CoRR}. \textbf{abs/2009.01884} (2020), https://arxiv.org/abs/2009.01884
\bibitem{crop}N Nithin Srivatsav, A. Crop Recommendation Dataset. (Kaggle,2020), https://www.kaggle.com/datasets/atharvaingle/crop-recommendation-dataset
\bibitem{bach2015pixel}Bach, S., Binder, A., Montavon, G., Klauschen, F., Müller, K. \& Samek, W. On pixel-wise explanations for non-linear classifier decisions by layer-wise relevance propagation. {\em PloS One}. \textbf{10}, e0130140 (2015)
\bibitem{kindermans2017learning}Kindermans, P., Schütt, K., Alber, M., Müller, K., Erhan, D., Kim, B. \& Dähne, S. Learning how to explain neural networks: Patternnet and patternattribution. {\em ArXiv Preprint ArXiv:1705.05598}. (2017)
\bibitem{zintgraf2017visualizing}Zintgraf, L., Cohen, T., Adel, T. \& Welling, M. Visualizing deep neural network decisions: Prediction difference analysis. {\em ArXiv Preprint ArXiv:1702.04595}. (2017)
\bibitem{kim2018interpretability}Kim, B., Wattenberg, M., Gilmer, J., Cai, C., Wexler, J., Viegas, F. \& Others Interpretability beyond feature attribution: Quantitative testing with concept activation vectors (tcav). {\em International Conference On Machine Learning}. pp. 2668-2677 (2018)
\bibitem{yuan2020xgnn}Yuan, H., Tang, J., Hu, X. \& Ji, S. Xgnn: Towards model-level explanations of graph neural networks. {\em Proceedings Of The 26th ACM SIGKDD International Conference On Knowledge Discovery & Data Mining}. pp. 430-438 (2020)
\bibitem{ribeiro2018anchors}Ribeiro, M., Singh, S. \& Guestrin, C. Anchors: High-Precision Model-Agnostic Explanations. {\em Proceedings Of The AAAI Conference On Artificial Intelligence}. \textbf{32} (2018), https://ojs.aaai.org/index.php/AAAI/article/view/11491
\bibitem{shap}Lundberg, S. \& Lee, S. A Unified Approach to Interpreting Model Predictions. {\em Proceedings Of The 31st International Conference On Neural Information Processing Systems}. pp. 4768-4777 (2017)
\bibitem{251526}Jagielski, M., Carlini, N., Berthelot, D., Kurakin, A. \& Papernot, N. High Accuracy and High Fidelity Extraction of Neural Networks. {\em 29th USENIX Security Symposium (USENIX Security 20)}. pp. 1345-1362 (2020,8), https://www.usenix.org/conference/usenixsecurity20/presentation/jagielski
\bibitem{dwork}Dwork, C., McSherry, F., Nissim, K. \& Smith, A. Calibrating noise to sensitivity in private data analysis. {\em Theory Of Cryptography: Third Theory Of Cryptography Conference, TCC 2006, New York, NY, USA, March 4-7, 2006. Proceedings 3}. pp. 265-284 (2006)
\bibitem{10.1145/3052973.3053009}Papernot, N., McDaniel, P., Goodfellow, I., Jha, S., Celik, Z. \& Swami, A. Practical Black-Box Attacks against Machine Learning. {\em Proceedings Of The 2017 ACM On Asia Conference On Computer And Communications Security}. pp. 506-519 (2017), https://doi.org/10.1145/3052973.3053009
\bibitem{10.1145/3287560.3287562}Milli, S., Schmidt, L., Dragan, A. \& Hardt, M. Model Reconstruction from Model Explanations. {\em Proceedings Of The Conference On Fairness, Accountability, And Transparency}. pp. 1-9 (2019), https://doi.org/10.1145/3287560.3287562
\bibitem{wang2018stealing}Wang, B. \& Gong, N. Stealing Hyperparameters in Machine Learning. {\em 2018 IEEE Symposium On Security And Privacy (SP)}. pp. 36-52 (2018)
\bibitem{brendel2018decisionbased}Brendel, W., Rauber, J. \& Bethge, M. Decision-Based Adversarial Attacks: Reliable Attacks Against Black-Box Machine Learning Models.  (2018)
\bibitem{papernot2016transferability}Papernot, N., McDaniel, P. \& Goodfellow, I. Transferability in machine learning: from phenomena to black-box attacks using adversarial samples. {\em ArXiv Preprint ArXiv:1605.07277}. (2016)
\bibitem{7943475}Shi, Y., Sagduyu, Y. \& Grushin, A. How to steal a machine learning classifier with deep learning. {\em 2017 IEEE International Symposium On Technologies For Homeland Security (HST)}. pp. 1-5 (2017)
\bibitem{orekondy2019knockoff}Orekondy, T., Schiele, B. \& Fritz, M. Knockoff nets: Stealing functionality of black-box models. {\em Proceedings Of The IEEE/CVF Conference On Computer Vision And Pattern Recognition}. pp. 4954-4963 (2019)
\bibitem{duddu2018stealing}Duddu, V., Samanta, D., Rao, D. \& Balas, V. Stealing neural networks via timing side channels. {\em ArXiv Preprint ArXiv:1812.11720}. (2018)
\bibitem{humbert2013addressing}Humbert, M., Ayday, E., Hubaux, J. \& Telenti, A. Addressing the concerns of the lacks family: quantification of kin genomic privacy. {\em Proceedings Of The 2013 ACM SIGSAC Conference On Computer & Communications Security}. pp. 1141-1152 (2013)
\bibitem{von2019re}Von Thenen, N., Ayday, E. \& Cicek, A. Re-identification of individuals in genomic data-sharing beacons via allele inference. {\em Bioinformatics}. \textbf{35}, 365-371 (2019)
\bibitem{humbert2015anonymizing}Humbert, M., Huguenin, K., Hugonot, J., Ayday, E. \& Hubaux, J. De-anonymizing genomic databases using phenotypic traits. {\em 15th Privacy Enhancing Technologies Symposium (PETS)}. \textbf{2015}, 99-114 (2015)
\bibitem{8806737}Juuti, M., Szyller, S., Marchal, S. \& Asokan, N. PRADA: Protecting Against DNN Model Stealing Attacks. {\em 2019 IEEE European Symposium On Security And Privacy (EuroS&P)}. pp. 512-527 (2019)
\bibitem{salem2018ml}Salem, A., Zhang, Y., Humbert, M., Berrang, P., Fritz, M. \& Backes, M. Ml-leaks: Model and data independent membership inference attacks and defenses on machine learning models. {\em ArXiv Preprint ArXiv:1806.01246}. (2018)
\bibitem{shokri2017membership}Shokri, R., Stronati, M., Song, C. \& Shmatikov, V. Membership inference attacks against machine learning models. {\em 2017 IEEE Symposium On Security And Privacy (SP)}. pp. 3-18 (2017)
\bibitem{ganju2018property}Ganju, K., Wang, Q., Yang, W., Gunter, C. \& Borisov, N. Property inference attacks on fully connected neural networks using permutation invariant representations. {\em Proceedings Of The 2018 ACM SIGSAC Conference On Computer And Communications Security}. pp. 619-633 (2018)
\bibitem{song2019overlearning}Song, C. \& Shmatikov, V. Overlearning reveals sensitive attributes. {\em ArXiv Preprint ArXiv:1905.11742}. (2019)
\bibitem{carlini2019secret}Carlini, N., Liu, C., Erlingsson, Ú., Kos, J. \& Song, D. The Secret Sharer: Evaluating and Testing Unintended Memorization in Neural Networks.. {\em USENIX Security Symposium}. \textbf{267} (2019)
\bibitem{zhang2020secret}Zhang, Y., Jia, R., Pei, H., Wang, W., Li, B. \& Song, D. The secret revealer: Generative model-inversion attacks against deep neural networks. {\em Proceedings Of The IEEE/CVF Conference On Computer Vision And Pattern Recognition}. pp. 253-261 (2020)
\bibitem{shokri2021privacy}Shokri, R., Strobel, M. \& Zick, Y. On the privacy risks of model explanations. {\em Proceedings Of The 2021 AAAI/ACM Conference On AI, Ethics, And Society}. pp. 231-241 (2021)
\bibitem{zhao2021exploiting}Zhao, X., Zhang, W., Xiao, X. \& Lim, B. Exploiting explanations for model inversion attacks. {\em Proceedings Of The IEEE/CVF International Conference On Computer Vision}. pp. 682-692 (2021)
\bibitem{Yan}Yan, A., Huang, T., Ke, L., Liu, X., Chen, Q. \& Dong, C. Explanation leaks: Explanation-guided model extraction attacks. {\em Information Sciences}. \textbf{632} pp. 269-284 (2023), https://www.sciencedirect.com/science/article/pii/S002002552300316X
\bibitem{Truong}Truong, J., Maini, P., Walls, R. \& Papernot, N. Data-Free Model Extraction. {\em CoRR}. \textbf{abs/2011.14779} (2020), https://arxiv.org/abs/2011.14779
\bibitem{kariyappa}Kariyappa, S. \& Qureshi, M. Defending against model stealing attacks with adaptive misinformation. {\em Proceedings Of The IEEE/CVF Conference On Computer Vision And Pattern Recognition}. pp. 770-778 (2020)
\bibitem{Miura}Miura, T., Hasegawa, S. \& Shibahara, T. MEGEX: Data-Free Model Extraction Attack against Gradient-Based Explainable AI. {\em CoRR}. \textbf{abs/2107.08909} (2021), https://arxiv.org/abs/2107.08909
\bibitem{aivodji}Aı̈vodji, U., Bolot, A. \& Gambs, S. Model extraction from counterfactual explanations. {\em ArXiv Preprint ArXiv:2009.01884}. (2020)
\bibitem{TrustOverIP}ToIP The ToIP Technology Architecture Specification. , https://trustoverip.org/our-work/technical-architecture/
\bibitem{SSI}Hendrickson, L. Your Guide to Self-Sovereign Identity (SSI).  (2024), https://www.identity.com/self-sovereign-identity
\bibitem{introToToIP}IP, T. Introduction to Trust Over IP.  (2021), https://trustoverip.org/wp-content/uploads/Introduction-to-ToIP-V2.0-2021-11-17.pdf
\bibitem{FLonAWS}Olivia Choudhury \& Ratan, U. Federated Learning on AWS with FedML: Health analytics without sharing sensitive data – Part 1.  (2023), https://aws.amazon.com/blogs/machine-learning/part-1-federated-learning-on-aws-with-fedml-health-analytics-without-sharing-sensitive-data/
\bibitem{startedwithNitro}AWS, A. Getting started: Hello enclave. , https://docs.aws.amazon.com/enclaves/latest/user/getting-started.html
\bibitem{takeout}Google Google Takeout. , https://takeout.google.com/%20
\bibitem{ToIPFoundation}ToIPFoundation Trust Over IP Foundation. , https://trustoverip.org/
\bibitem{VerifiableCredentials}W3 Verifiable Credentials Data Model v2.0. , https://www.w3.org/TR/vc-data-model-2.0/
\bibitem{podgorelec2022digital}Podgorelec, B., Alber, L. \& Zefferer, T. What is a (digital) identity wallet? a systematic literature review. {\em 2022 IEEE 46th Annual Computers, Software, And Applications Conference (COMPSAC)}. pp. 809-818 (2022)
\bibitem{openwallet2023}OpenWallet Foundation OpenWallet Foundation. (https://openwallet.foundation/,2023)
\bibitem{mydex}Mydex.org Mydex Community Interest Company takes a Human Rights Approach to Personal Data collection, storage and sharing.. , https://mydex.org
\bibitem{Sovrin}Sovren.org Global public registry for DIDs Trust anchor for Verifiable Credentials. , https://sovrin.org
\bibitem{uport}UPort uPort - Open Identity System for the Decentralized Web. (ConsenSys AG,2023), https://www.uport.me/
\bibitem{Dataswyft}Dataswyft.io dataswyft, Personal Data Accounts. , https://www.dataswyft.io/concepts/personal-data-account
\bibitem{fortunebusinessinsights2023}Fortune Business Insights Data Privacy Software Market . (Fortune Business Insights,2023), https://www.fortunebusinessinsights.com/press-release/global-data-privacy-software-market-10655
\bibitem{make3020017}Papadopoulos, P., Abramson, W., Hall, A., Pitropakis, N. \& Buchanan, W. Privacy and Trust Redefined in Federated Machine Learning. {\em Machine Learning And Knowledge Extraction}. \textbf{3}, 333-356 (2021), https://www.mdpi.com/2504-4990/3/2/17
\bibitem{metriport}Metriport Medical API. , https://www.metriport.com/medical
\bibitem{sleepStudy}Tharmalingam, L. Sleep Health and Lifestyle Dataset. , https://www.kaggle.com/datasets/uom190346a/sleep-health-and-lifestyle-dataset
\bibitem{costan2016intel}Costan, V. \& Devadas, S. Intel SGX Explained. {\em IACR Cryptol. EPrint Arch.}. \textbf{2016}, 1-118 (2016)
\bibitem{qi2020stanza}Qi, P., Zhang, Y., Zhang, Y., Bolton, J. \& Manning, C. Stanza: A Python natural language processing toolkit for many human languages. {\em ArXiv Preprint ArXiv:2003.07082}. (2020)
\bibitem{reimers2019BERT}Reimers, N. \& Gurevych, I. Sentence-BERT: Sentence Embeddings using Siamese BERT-Networks. {\em ArXiv Preprint ArXiv:1908.10084}. (2019), https://arxiv.org/abs/1908.10084
\bibitem{emp-toolkit}Wang, X., Malozemoff, A. \& Katz, J. EMP-toolkit: Efficient MultiParty computation toolkit.  (2016)
\bibitem{fresco}Alexandra Institute FRESCO: A FRamework for Efficient Secure COmputation.  (2015)
\bibitem{w3c_vc_2022}W3C Verifiable Credentials Data Model v2.0. (World Wide Web Consortium,2022), https://www.w3.org/TR/vc-data-model-2.0/
\bibitem{fredrikson2015model}Fredrikson, M., Jha, S. \& Ristenpart, T. Model inversion attacks that exploit confidence information and basic countermeasures. {\em Proceedings Of The 22nd ACM SIGSAC Conference On Computer And Communications Security}. pp. 1322-1333 (2015)
\bibitem{narayanan2008robust}Narayanan, A. \& Shmatikov, V. Robust de-anonymization of large sparse datasets. {\em 2008 IEEE Symposium On Security And Privacy (sp 2008)}. pp. 111-125 (2008)
\bibitem{FERPA}U.S. Department of Education Family Educational Rights and Privacy Act (FERPA). (https://www.ecfr.gov/current/title-34/subtitle-A/part-99,2018), 20 U.S.C. § 1232g; 34 CFR Part 99
\bibitem{goldwasser2019knowledge}Goldwasser, S., Micali, S. \& Rackoff, C. The knowledge complexity of interactive proof-systems. {\em Providing Sound Foundations For Cryptography: On The Work Of Shafi Goldwasser And Silvio Micali}. pp. 203-225 (2019)
\bibitem{scalemamba}Aly, A., Cozzo, D., Keller, M., Orsini, E., Rotaru, D., Scholl, P., Smart, N. \& Wood, T. SCALE-MAMBA Software.  (2018)
\bibitem{mp-spdz}Keller, M. MP-SPDZ: A Versatile Framework for Multi-Party Computation. {\em Proceedings Of The 2020 ACM SIGSAC Conference On Computer And Communications Security}. (2020), https://doi.org/10.1145/3372297.3417872
\bibitem{mcmahan2017communication}McMahan, B., Moore, E., Ramage, D., Hampson, S. \& Arcas, B. Communication-efficient learning of deep networks from decentralized data. {\em Artificial Intelligence And Statistics}. pp. 1273-1282 (2017)
\bibitem{camenisch2001efficient}Camenisch, J. \& Lysyanskaya, A. An efficient system for non-transferable anonymous credentials with optional anonymity revocation. {\em International Conference On The Theory And Applications Of Cryptographic Techniques}. pp. 93-118 (2001)
\bibitem{chen2004new}Chen, X., Orlowska, M. \& Li, X. A new framework of privacy preserving data sharing. {\em Proc. Of The 4th IEEE ICDM Workshop: Privacy And Security Aspects Of Data Mining. IEEE Computer Society}. pp. 47-56 (2004)
\bibitem{zheng2018scalable}Zheng, B., Zhu, L., Shen, M., Gao, F., Zhang, C., Li, Y. \& Yang, J. Scalable and privacy-preserving data sharing based on blockchain. {\em Journal Of Computer Science And Technology}. \textbf{33} pp. 557-567 (2018)
\bibitem{dong2014achieving}Dong, X., Yu, J., Luo, Y., Chen, Y., Xue, G. \& Li, M. Achieving an effective, scalable and privacy-preserving data sharing service in cloud computing. {\em Computers & Security}. \textbf{42} pp. 151-164 (2014)
\bibitem{dunning2012privacy}Dunning, L. \& Kresman, R. Privacy preserving data sharing with anonymous ID assignment. {\em IEEE Transactions On Information Forensics And Security}. \textbf{8}, 402-413 (2012)
\bibitem{aggarwal2008general}Aggarwal, C. \& Yu, P. A general survey of privacy-preserving data mining models and algorithms. (Springer,2008)
\bibitem{google}Google LLC Google. (https://www.google.com/,2023)
\bibitem{gdpr2016}European Parliament and Council of the European Union Regulation (EU) 2016/679 of the European Parliament and of the Council of 27 April 2016 on the protection of natural persons with regard to the processing of personal data and on the free movement of such data, and repealing Directive 95/46/EC (General Data Protection Regulation). (https://eur-lex.europa.eu/eli/reg/2016/679/oj,2016)
\bibitem{ccpa2018}California State Legislature California Consumer Privacy Act of 2018. (https://about.clearancejobs.com/ccpa,2018)
\bibitem{ethereum}Ethereum Foundation Ethereum. (https://ethereum.org/,2023)
\bibitem{dmitrienko2014security}Dmitrienko, A., Liebchen, C., Rossow, C. \& Sadeghi, A. On the (in) security of mobile two-factor authentication. {\em Financial Cryptography And Data Security: 18th International Conference, FC 2014, Christ Church, Barbados, March 3-7, 2014, Revised Selected Papers 18}. pp. 365-383 (2014)
\bibitem{rfc4226}M'Raihi, D., Bellare, M., Hoornaert, F., Naccache, D. \& Ranen, O. HOTP: An HMAC-Based One-Time Password Algorithm. (RFC Editor,2005,12), https://www.rfc-editor.org/info/rfc4226
\bibitem{amazon}Amazon.com, Inc. Amazon. (https://www.amazon.com/,2023)
\bibitem{yao1982protocols}Yao, A. Protocols for secure computations. {\em 23rd Annual Symposium On Foundations Of Computer Science (sfcs 1982)}. pp. 160-164 (1982)
\bibitem{dwork2014algorithmic}Dwork, C. \& Roth, A. The algorithmic foundations of differential privacy. {\em Foundations And Trends In Theoretical Computer Science}. \textbf{9}, 211-407 (2014)
\bibitem{ben2018scalable}Ben-Sasson, E., Bentov, I., Horesh, Y. \& Riabzev, M. Scalable, transparent, and post-quantum secure computational integrity. {\em IACR Cryptol. EPrint Arch.}. \textbf{2018} pp. 46 (2018)
\bibitem{cavoukian2009privacy}Cavoukian, A. Privacy by design: The 7 foundational principles. {\em Information And Privacy Commissioner Of Ontario, Canada}. \textbf{5} pp. 12 (2009)
\bibitem{borges2015ecdsa}Borges, F., Moreira, M. \& Ferreira, R. ECDSA (Elliptic Curve Digital Signature Algorithm). {\em 6º CONTECSI-International Conference On Information Systems And Technology Management}. (2015)
\bibitem{boneh2004short}Boneh, D., Boyen, X. \& Shacham, H. Short group signatures. {\em Annual International Cryptology Conference}. pp. 41-55 (2004)
\bibitem{au2006constant}Au, M., Susilo, W. \& Mu, Y. Constant-size dynamic k-TAA. {\em Security And Cryptography For Networks: 5th International Conference, SCN 2006, Maiori, Italy, September 6-8, 2006. Proceedings 5}. pp. 111-125 (2006)
\bibitem{camenisch2016anonymous}Camenisch, J., Drijvers, M. \& Lehmann, A. Anonymous attestation using the strong diffie hellman assumption revisited. {\em Trust And Trustworthy Computing: 9th International Conference, TRUST 2016, Vienna, Austria, August 29-30, 2016, Proceedings 9}. pp. 1-20 (2016)
\bibitem{goldreich1998secure}Goldreich, O. Secure multi-party computation. {\em Manuscript. Preliminary Version}. \textbf{78}, 1-108 (1998)
\bibitem{bonneau2015sok}Bonneau, J., Miller, A., Clark, J., Narayanan, A., Kroll, J. \& Felten, E. SoK: Research perspectives and challenges for bitcoin and cryptocurrencies. {\em 2015 IEEE Symposium On Security And Privacy}. pp. 104-121 (2015)
\bibitem{parno2013pinocchio}Parno, B., Howell, J., Gentry, C. \& Raykova, M. Pinocchio: Nearly practical verifiable computation. {\em 2013 IEEE Symposium On Security And Privacy}. pp. 238-252 (2013)
\bibitem{kosba2016hawk}Kosba, A., Miller, A., Shi, E., Wen, Z. \& Papamanthou, C. Hawk: The blockchain model of cryptography and privacy-preserving smart contracts. {\em 2016 IEEE Symposium On Security And Privacy (SP)}. pp. 839-858 (2016)
\bibitem{tianxi_vldb}Ji, T., Li, P., Yilmaz, E., Ayday, E., Ye, Y. \& Sun, J. Differentially Private Binary- and Matrix-Valued Data Query. {\em Proceedings Of The International Conference On Very Large Data Bases (VLDB)}. pp. 849-862 (2021)
\bibitem{leonard_amia}Dervishi, L., Wang, X., Li, W., Halimi, A., J. Vaidya, X. \& Ayday, E. Facilitating Federated Genomic Data Analysis by Identifying Record Correlations while Ensuring Privacy. {\em Proceedings Of American Medical Informatics Association (AMIA) Annual Symposium}. (2022)
\bibitem{xinyue_amia}Wang, X., Dervishi, L., Li, W., Jiang, X., Ayday, E. \& Vaidya, J. Efficient Federated Kinship Relationship Identification. {\em Proceedings Of American Medical Informatics Association (AMIA) Annual Symposium}. (2023)
\bibitem{leonard_ismb}Dervishi, L., Li, W., Halimi, A., Jiang, X., Vaidya, J. \& Ayday, E. Privacy Preserving Population Stratification for Collaborative Genomic Research. {\em Proceedings Of Intelligent Systems For Molecular Biology (ISMB)}. (2023)
\bibitem{rieke2020future}Rieke, N., Hancox, J., Li, W., Milletari, F., Roth, H., Albarqouni, S., Bakas, S., Galtier, M., Landman, B., Maier-Hein, K. \& Others The future of digital health with federated learning. {\em NPJ Digital Medicine}. \textbf{3}, 1-7 (2020)
\bibitem{troncoso2007pripayd}Troncoso, C., Danezis, G., Kosta, E. \& Preneel, B. Pripayd: privacy friendly pay-as-you-drive insurance. {\em Proceedings Of The 2007 ACM Workshop On Privacy In Electronic Society}. pp. 99-107 (2007)
\bibitem{yilmaz_ayday}Yilmaz, E. \& Ayday, E. Probabilistic Fingerprinting Scheme for Correlated Data. {\em IFIP Annual Conference On Data And Applications Security And Privacy, Springer, 2023, Pp. 69–90}. (2023)
\bibitem{alserr_kale}Alserr, N., G. Kale, O., Tastan, O. \& Ayday, E. Tuning privacy-utility tradeoff in genomic studies using selective SNP hiding. {\em Asia-Pacific Bioinformatics Conference}. (2023)
\bibitem{tianxi_ndss}Ji, T., Ayday, E., Yilmaz, E. \& Li, P. Differentially-Private Fingerprinting of Relational Databases. {\em Proceedings Of The Annual Network & Distributed System Security Symposium – NDSS}. (2023)
\bibitem{ji_ayday}Ji, T., Ayday, E., Yilmaz, E. \& Li, P. Differentially-Private Fingerprinting of Relational Databases. {\em ArXiv Preprint ArXiv:2109.02768, 2021.}. (2021)
\bibitem{jing_ayday}Jiang, Y., Yilmaz, E. \& Ayday, E. Robust Fingerprint of Location Trajectories Under Differential Privacy. {\em Privacy Enhancing Technologies Symposium, NIH Public Access, 2023, P. 5}. (2023)
\bibitem{ji_ayday_2}T. Ji \& Li, P. Robust fingerprinting of genomic databases. {\em Bioinformatics, Vol. 38, No. Supplement_1, Pp. I143–i152, 2022}. (2022)
\bibitem{halimi_et_al}Al, A. Privacy-preserving and efficient verification of the outcome in genome-wide association studies. {\em Privacy Enhancing Technologies Symposium, NIH Public Access, 2022, P. 732}. (2022)
\bibitem{wang_dervishi}Wang, X., Dervishi, L., Li, W., Ayday, E., Jiang, X. \& Vaidya, J. Privacy-preserving federated genome-wide association studies via dynamic sampling. {\em Bioinformatics, Vol. 39, No. 10, P. Btad639, 2023}. (2023)
\bibitem{zhu_ayday}Zhu, X., Ayday, E. \& Vitenberg, R. A privacy-preserving framework for conducting genome-wide association studies over outsourced patient data. {\em IEEE Transactions On Dependable And Secure Computing, 2022}. (2022)
\bibitem{gao_yoo}Gao, K., Yoo, Y. \& Schecter, A. Models as Social Actors in the Diffusion of AI Innovations: A Multilayer, Heterogeneous, Dynamic Network Perspective.  (2023), https://aisel.aisnet.org/icis2023/diginnoventren/diginnoventren/6/
\bibitem{homer2008resolving}Homer, N., Szelinger, S., Redman, M., Duggan, D., Tembe, W., Muehling, J., Pearson, J., Stephan, D., Nelson, S. \& Craig, D. Resolving individuals contributing trace amounts of DNA to highly complex mixtures using high-density SNP genotyping microarrays. {\em PLoS Genetics}. \textbf{4}, e1000167 (2008)
\bibitem{yuzhou_arxiv_2024}Jiang, Y., Ji, T., Li, P. \& Ayday, E. Reproducibility-Oriented and Privacy-Preserving Genomic Dataset Sharing.  (2024), https://arxiv.org/abs/2209.06327
\bibitem{similar_patiens_arxiv}Zhu, X., Ayday, E., Vitenberg, R. \& Veeraragavan, N. Privacy-Preserving Search for a Similar Genomic Makeup in the Cloud. {\em IEEE Transactions On Dependable And Secure Computing}. (2021)
\bibitem{Dwork2014-fc}Dwork, C. \& Roth, A. The Algorithmic Foundations of Differential Privacy. {\em Found. Trends Theor. Comput. Sci.}. \textbf{9}, 211-407 (2014)
\bibitem{Tatton2022ShareTraceCT}Tatton, R., Ayday, E., Yoo, Y. \& Halimi, A. ShareTrace: Contact Tracing with the Actor Model. {\em 2022 IEEE International Conference On E-health Networking, Application & Services (HealthCom)}. pp. 13-18 (2022)
\bibitem{ayday_BCB21}Ayday, E., Yoo, Y. \& Halimi, A. ShareTrace: an iterative message passing algorithm for efficient and effective disease risk assessment on an interaction graph. {\em Proceedings Of The 12th ACM Conference On Bioinformatics, Computational Biology, And Health Informatics}. (2021), https://doi.org/10.1145/3459930.3469553
\bibitem{americafirstpolicy2023}America First Policy Institute Learning and Employment Records: A Pathway for Restoring America’s Workforce.  (2023), https://americafirstpolicy.com/assets/uploads/files/learning-and-employment-records-a-pathway-for-restoring-americas-workforce.pdf
\bibitem{zeng2023pandalm}Zeng, W., Nie, X., Sun, T., Wu, Z. \& Lyu, L. PandaLM: An Automatic Evaluation Benchmark for LLM Instruction Tuning Optimization. {\em ArXiv Preprint ArXiv:2302.09938}. (2023)
\bibitem{IJCRT2021study}Mahajan, A. \& Kapoor, S. A Study of Issues in Job Portals. {\em International Journal Of Creative Research Thoughts (IJCRT)}. \textbf{9}, 1476-1480 (2021), https://ijcrt.org/papers/IJCRT2104174.pdf
\bibitem{sabet2024course}Sabet, A., Bana, S., Yu, R. \& Frank, M. Course-Skill Atlas: A national longitudinal dataset of skills taught in U.S. Higher education curricula. {\em ArXiv}. (2024), https://arxiv.org/abs/2404.13163
\bibitem{BPC}BPCnet CWRU - BPC. , https://plans.bpcnet.org/
\bibitem{acquistiEconomicsPrivacyCrossroads2022}Acquisti, A. The Economics of Privacy at a Crossroads. {\em NBER Chapters}. (2022), https://www.nber.org/system/files/chapters/c14785/revisions/c14785.rev1.pdf
\bibitem{cennamoDigitalPlatformsRegulation2022}Cennamo, C., Kretschmer, T., Constantinides, P., Alaimo, C. \& Santalo, J. Digital Platforms Regulation: An Innovation-Centric View of the EU’s Digital Markets Act. {\em Journal Of European Competition Lawy & Practice}. (2022,7,1), https://dx.doi.org/10.2139/ssrn.4152120
\bibitem{coaseProblemSocialCost1960}Coase, R. The Problem of Social Cost. {\em The Journal Of Law And Economics}. \textbf{3} pp. 1-44 (1960), https://app.readcube.com/library/9325db16-ddab-4808-a4d1-0a331744be80/item/20a33242-8210-46f6-81f3-92f5c598c29c
\bibitem{gregoryCOOPERATIONSTRANGERSALGORITHMIC2024}Gregory, R. COOPERATION AMONG STRANGERS: ALGORITHMIC ENFORCEMENT OF RECIPROCAL EXCHANGE WITH BLOCKCHAIN-BASED SMART CONTRACTS. {\em Academy Of Management Review}. (2024)
\bibitem{gregoryRoleArtificialIntelligence2021}Gregory, R., Henfridsson, O., Kaganer, E. \& Kyriakou, H. The Role of Artificial Intelligence and Data Network Effects for Creating User Value. {\em Academy Of Management Review}. \textbf{46}, 534-551 (2021,7), http://journals.aom.org/doi/full/10.5465/amr.2019.0178
\bibitem{hartIncompleteContractsOwnership2007}Hart, O. \& Moore, J. Incomplete Contracts and Ownership: Some New Thoughts. {\em American Economic Review}. \textbf{97}, 182-186 (2007)
\bibitem{tuckerEconomicsPrivacyAgenda2023}Tucker, C. The Economics of Privacy: An Agenda.  (2023)
\bibitem{jonesNonrivalryEconomicsData2020}Jones, C. \& Tonetti, C. Nonrivalry and the Economics of Data. {\em American Economic Review}. \textbf{110}, 2819-58 (2020), https://www.aeaweb.org/articles?id=10.1257/aer.20191330
\bibitem{karhuPOSITIVENEGATIVEAMPLIFIED2024}Karhu, K. \& Heiskala, M. POSITIVE, NEGATIVE, AND AMPLIFIED NETWORK EXTERNALITIES IN PLATFORM MARKETS. {\em Academy Of Management Perspectives}. (2024)
\bibitem{bernal2019privacy}Bernal Bernabe, J., Canovas, J., Hernandez-Ramos, J., Torres Moreno, A. \& Skarmeta, A. Privacy-Preserving Solutions for Blockchain: Review and Challenges. {\em IEEE Access}. \textbf{7} pp. 164908-164940 (2019), https://ieeexplore.ieee.org/document/8888155
\bibitem{synergizing2024privacy}Unknown, A. Synergizing Privacy and Utility in Data Analytics Through Advanced Techniques. {\em ArXiv Preprint ArXiv:2404.16241}. (2024)
\bibitem{AWS-ECS}AWS, A. Amazon Elastic Container Service. , https://aws.amazon.com/ecs/
\bibitem{DIDs}DIDComm Decentralized Identifiers (DIDs). , https://www.w3.org/TR/did-core/
\bibitem{DIDComm}DIDComm DIDComm Messaging. , https://identity.foundation/didcomm-messaging/spec/v2.1/
\bibitem{alazab2024privacy}Alazab, M., Gadekallu, T., Pham, Q., Maddikunta, P., Bhattacharya, S., Piran, M. \& Hossain, M. Privacy and Security in Distributed Learning: A Review of Challenges, Solutions, and Open Research Issues. {\em IEEE Transactions On Industrial Informatics}. (2024), https://ieeexplore.ieee.org/document/10278413
\bibitem{ABAC}Amazon-AWS Attribute-Based Access Control (ABAC) for AWS. , https://aws.amazon.com/identity/attribute-based-access-control
\bibitem{AWSNitroEnclaves}Amazon.com AWS Nitro Enclaves: Create additional isolation to further protect highly sensitive data within EC2 instances. , https://aws.amazon.com/ec2/nitro/nitro-enclaves/
\bibitem{aslan2023}Aslan, Ö., Aktuğ, S., Ozkan-Okay, M., Yilmaz, A. \& Akin, E. A Comprehensive Review of Cyber Security Vulnerabilities, Threats, Attacks, and Solutions. {\em Electronics}. \textbf{12} (2023), https://www.mdpi.com/2079-9292/12/6/1333
\bibitem{whatIsNitro}AWS, A. What is AWS Nitro Enclaves?. , https://docs.aws.amazon.com/enclaves/latest/user/nitro-enclave.html
\bibitem{battiston2023}Battiston, I. \& Boncz, P. Improving Data Minimization through Decentralized Data Architectures. {\em ArXiv}. \textbf{2312.12923} (2023), https://arxiv.org/abs/2312.12923
\bibitem{ben2014succinct}Ben-Sasson, E., Chiesa, A., Tromer, E. \& Virza, M. Succinct non-interactive zero knowledge for a von Neumann architecture. {\em 23rd USENIX Security Symposium (USENIX Security 14)}. pp. 781-796 (2014)
\bibitem{bunz2018bulletproofs}B"unz, B., Bootle, J., Boneh, D., Poelstra, A., Wuille, P. \& Maxwell, G. Bulletproofs: Short proofs for confidential transactions and more. {\em 2018 IEEE Symposium On Security And Privacy (SP)}. pp. 315-334 (2018)
\bibitem{dataswift}Dataswift Dataswift - Personal Data Accounts. (Dataswift Ltd.,2023), https://dataswift.io/
\bibitem{digime}Digi.me digi.me - Your Data, Your Way. (digi.me Ltd.,2023), https://digi.me/
\bibitem{dwork2006differential}Dwork, C. Differential privacy. {\em International Colloquium On Automata, Languages, And Programming}. pp. 1-12 (2006)
\bibitem{databank}Fernández, M., Franch Tapia, A., Jaimunk, J., Martinez Chamorro, M. \& Thuraisingham, B. A Data Access Model for Privacy-Preserving Cloud-IoT Architectures. {\em Proceedings Of The 25th ACM Symposium On Access Control Models And Technologies}. pp. 191-202 (2020), https://doi.org/10.1145/3381991.3395610
\bibitem{groth2016size}Groth, J. On the size of pairing-based non-interactive arguments. {\em Annual International Conference On The Theory And Applications Of Cryptographic Techniques}. pp. 305-326 (2016)
\bibitem{latupeirissa2024}Latupeirissa, J., Dewi, N., Prayana, I., Srikandi, M., Ramadiansyah, S. \& Pramana, I. Transforming Public Service Delivery: A Comprehensive Review of Digitization Initiatives. {\em Sustainability}. \textbf{16}, 2818 (2024), https://www.mdpi.com/2071-1050/16/7/2818
\bibitem{meeco}Meeco Meeco: Enterprise Infrastructure for the Personal Data Economy. (https://www.meeco.me/), Accessed: 2024-12-03
\bibitem{mireshghallah2021privacy}Mireshghallah, F., Lundgren, M., Asghari, P., Ren, S., Kuzmanovic, A. \& Nilizadeh, S. Privacy-Preserving Machine Learning: Methods, Challenges, and Directions. {\em ArXiv Preprint ArXiv:2108.04417}. (2021)
\bibitem{databox}Mortier, R., Zhao, J., Crowcroft, J., Wang, L., Li, Q., Haddadi, H., Amar, Y., Crabtree, A., Colley, J., Lodge, T., Brown, T., McAuley, D. \& Greenhalgh, C. Personal Data Management with the Databox: What's Inside the Box?. {\em Proceedings Of The 2016 ACM Workshop On Cloud-Assisted Networking}. pp. 49-54 (2016), https://doi.org/10.1145/3010079.3010082
\bibitem{openpds}Openpds Openpds, Personal Data with Privacy. , https://openpds.media.mit.edu
\bibitem{personaldataio}PersonalData.IO Home - PersonalData.IO. (https://personaldata.io/en/home-en/), Accessed: 2024-12-03
\bibitem{ppds}Singh, B., Carminati, B. \& Ferrari, E. Privacy-Aware Personal Data Storage (P-PDS): Learning how to Protect User Privacy from External Applications. {\em IEEE Transactions On Dependable And Secure Computing}. \textbf{18}, 889-903 (2021)
\bibitem{Solid}Solid Solid: Your data, your choice.  (0), https://solidproject.org
\bibitem{wikipedia2021gdpr}Wikipedia contributors General Data Protection Regulation. (https://en.wikipedia.org/wiki/General_Data_Protection_Regulation,2021), Accessed: Mar 30, 2025
\bibitem{emre_codaspy}Yilmaz, E., T.Ji, Ayday, E. \& P.Li Genomic Data Sharing under Dependent Local Differential Privacy. {\em Proceedings Of ACM Conference On Data And Application Security And Privacy (CODASPY)}. (2022)


==> sections/acknowledgment.tex <==
\vspace{-2 mm}
\section{Acknowledgments}
\vspace{-2 mm}

This research was supported in part by the National Science Foundation (NSF) under awards OAC-2112606 and 2427505.  
